Deconstructing Sentimental Stack Overflow Posts Through Interviews: Exploring the Case of Software Testing

The analysis of sentimental posts about software testing on Stack Overflow reveals that motivation and commitment of developers to use software testing methods is not only influenced by tools and technology. Rather, attitudes are also influenced by socio-technical factors. No prior studies have attempted to talk with Stack Overflow users about the sentimental posts that they write, yet, this is crucial to understand their experiences of which their post is only a fragment. As such, this study explores the precursors that make developers write sentimental posts about software testing on Stack Overflow. Through semi-structured interviews, we reconstruct the individual experiences of Stack Overflow users leading to sentimental posts about testing. We use the post as an anchor point to explore the events that lead to it and how users moved on in the meantime. Using strategies from socio-technical grounded theory (STGT), we derive hypotheses about the socio-technical factors that cause sentiment towards software testing.

==> ccs.tex <==
% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
\begin{CCSXML}
\end{CCSXML}

\ccsdesc[300]{Software and its engineering~Programming teams}
\ccsdesc[300]{Human-centered computing~Natural language interfaces}
\ccsdesc[100]{Social and professional topics~Cultural characteristics}
\ccsdesc[100]{Computing methodologies~Simulation evaluation}



==> keywords.tex <==
%! TEX root = chase-2023-RR.tex
%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
%\keywords{TODO}


==> variables.tex <==
%! TEX root = chase-2023-RR.tex
\section{variables}
%%  * Independent Variable(s) and their operationalization
%%  * Dependent Variable(s) and their operationalization
%%    (e.g., time to solve a specified task)
%%  * Confounding Variable(s) and how their effect will be controlled
%%    (e.g., species type (Vulcan, Human, Tribble)
%%    might be a confounding factor;
%%    we control for it by separating our sample
%%    additionally into Human/Non-Human
%%    and using an ANOVA (normal distribution)
%%    or Friedman (non-normal distribution)
%%    to distill its effect).
%% For each variable, you should give:
%%  * name (e.g., presence of family)
%%  * abbreviation (if you intend to use one)
%%  * description (whether the family of the crew members travels on board)
%%  * scale type (nominal: either the family is present or not)
%%  * operationalization (crew members without family on board vs.
%%    crew members with family onboard)
TODO

